Pairwise Symmetry Reasoning for Multi-Agent Path Finding Search

Multi-Agent Path Finding (MAPF) is a challenging combinatorial problem that asks us to plan collision-free paths for a team of cooperative agents. In this work, we show that one of the reasons why MAPF is so hard to solve is due to a phenomenon called pairwise symmetry, which occurs when two agents have many different paths to their target locations, all of which appear promising, but every combination of them results in a collision. We identify several classes of pairwise symmetries and show that each one arises commonly in practice and can produce an exponential explosion in the space of possible collision resolutions, leading to unacceptable runtimes for current state-of-the-art (bounded-sub)optimal MAPF algorithms. We propose a variety of reasoning techniques that detect the symmetries efficiently as they arise and resolve them by using specialized constraints to eliminate all permutations of pairwise colliding paths in a single branching step. We implement these ideas in the context of the leading optimal MAPF algorithm CBS and show that the addition of the symmetry reasoning techniques can have a dramatic positive effect on its performance - we report a reduction in the number of node expansions by up to four orders of magnitude and an increase in scalability by up to thirty times. These gains allow us to solve to optimality a variety of challenging MAPF instances previously considered out of reach for CBS.

==> disjoint.tex <==
\section{Disjoint Symmetry-Breaking Constraints}
\label{sec:disjoint}

\jl{Introduce positive barrier constraint and positive range constraint.
They induce overhead in the low-level search but seldom reduce the size of the CT tree.
We need to explain the reason here carefully.}


==> epea.tex <==
\subsection{Comparison with Other Search-Based MAPF Algorithms}\label{sec:epea}
